VoroDuce: Massively Parallel 3D Voronoi Simplification with Volume-Aware Edge Collapse

3D Voronoi diagrams provide a powerful mathematical framework for representing volumetric functions and geometry with applications to Materials Science, Biology, Simulation and Astrophysics. However, accurately resolving fine structures often requires millions of cells, imposing severe computational and memory constraints. Traditional mesh decimation or point cloud simplification techniques fail to account for the effects re-meshing has on neighbouring cells. In this work, we formalize the Voronoi reduction problem and propose a greedy edge-collapsing algorithm on the dual Delaunay tetrahedralisation that accounts for changes in the local geometry. Further, we demonstrate a novel volumetric error approximation technique that models convex cell intersections as truncated prismatoids, circumventing computationally prohibitive exact volume calculations and enabling massive GPU parallelization. Evaluations across Synthetic, Medicine and Material Science data demonstrate that VoroDuce decimates models with up to a million primitives, successfully compressing the representation while preserving the underlying data better than naive decimation approaches.

==> Sections/Approximating_Intersection_Volumes_Legacy.tex <==
\paragraph{Approximating Neighbour Intersection Volumes}


Examining the intersections of neighbour cells (Equations \ref{eq1} to \ref{eq3}) after merging with the original cell pair of an edge collapse in Figure \ref{fig:voronoi_volume_costs}, we notice an interesting pattern in the intersection with neighbour cells: While the intersection of two convex cells is a new convex cell with arbitrary vertex count, in the majority of cases, the intersection with neighbours after an edge collapse results in cells with specifically 4 or 3 vertices. We differentiate four different cases:
\begin{itemize}
    \item[\ding{172}] The intersection is a quadrangle, where the area is spanned between an inner red and an outer blue line segment.
    \item[\ding{173}] A red and blue line segment intersect, creating two triangles.
    \item[\ding{174}] The intersection is a triangle formed by a blue line segment and a new point (green).
    \item[\ding{175}] The intersection is the convex hull of a red and blue line segment and at least one new point (green). 
\end{itemize}

For 2 points $\mathbf{x}_i, \mathbf{x}_j$ that are merging to $\mathbf{x}_{new}$, let $k \in \mathcal{N}(i)$. In case 1, $\mathcal{F}_{k, new}$ and $\mathcal{F}_{k, i}$ do not intersect, meaning $Vol(\hat{V}_{new} \cap V_k) = 0$. As such, for the cost computation, we only need to find $Vol(V_i \cap \hat{V}_k)$, which is itself a convex cell. There are two faces of $Vol(V_i \cap \hat{V}_k)$ we can compute directly: $\mathcal{F}_{k, new}$ and $\mathcal{F}_{k, i}$. 
\begin{equation}
    \mathcal{F}_{k, new} = \Pi_{\mathbf{x}_k, \mathbf{x}_{new}} \cap \bigcap_{j \in \mathcal{N}(k) \cap \mathcal{N}(new)} \Pi^+_{\mathbf{x}_i, \mathbf{x}_n}
\end{equation}

\begin{equation}
    \mathcal{F}_{k, i} = \Pi_{\mathbf{x}_k, \mathbf{x}_{i}} \cap \bigcap_{j \in \mathcal{N}(k) \cap \mathcal{N}(i)} \Pi^+_{\mathbf{x}_i, \mathbf{x}_n}
\end{equation}

(cf. Equation \ref{Eq:Face})

Thesis: If $|\mathcal{F}_{k, i}| = |\mathcal{F}_{k, new}|$, then \\

Question 1: When is $Vol(V_i \cap \hat{V}_k)= Vol(\hat{V}_k) - Vol(V_k)$? \\
Question 2: When is $\hat{V}_k =\bigcap_{l\in \mathcal{N}(k) \setminus } \Pi^+_{\mathbf{x}_k, \mathbf{x}_l}$? \\



For 

In 3D, the blue and red line segments each represent a convex polygon (the shared face with a neighbour before and after the merge respectively), which we will refer to as $\mathcal{F}_{orig}$ and $\mathcal{F}_{new}$ respectively. Let $\mathbf{x}_{orig}$ denote a point neighboured to $\mathbf{x}_{n}$ that is merged to form $\mathbf{x}_{new}$. The face $\mathcal{F}_{new}$  








As such, Case \ding{172} in 3D means that the interface $\mathcal{F}_{orig}$ simply shifted to $\mathcal{F}_{new}$ without changing the number of neighbour cells. Its change in volume can thus be represented exactly as a truncated prismatoid (the volume between $\mathcal{F}_{orig}$ and $\mathcal{F}_{new}$). In Case 2, the original and new cell boundaries intersect, defining one gained and one lost volume, both of which can be described by a truncated prismatoid.
Computing the volume of a truncated prismatoid is a very efficient and parallelizable operation given its vertices (See Supplemental X). Therefore we can reduce the task of finding the intersection volumes for these cases to finding $\mathcal{F}_{orig}$ and $\mathcal{F}_{new}$.

Case 3 represents cells which are no longer neighboured to the merged cell. Therefore, they lose one of the faces that define it, creating a general convex cell. Computing the exact shape and volume of these cells would be severely inefficient, so we instead approximate these cases as pyramids with base polygon $\mathcal{F}_{orig}$ and apex $c + normal(\mathcal{F}_{orig}) \cdot \min_t{c + t \cdot normal(\mathcal{F}_{orig}) \in \mathcal{H}}$.

Notably, 
Case 3 implies that the Delaunay edge between a neighbour and the merged cell is removed. According to Euler's formula, the number of Delaunay edges must remain constant after the merge (except for the merged edges). Thus, the edge does not vanish, but instead \textit{flips} to different neighbour cells that were previously unconnected. The specific edge flip from the 2D example is illustrated in Figure~\ref{fig:edgeflips} and results in Case 4: For the cells with the newly created Delaunay edge, the change in volume is no longer a quadrangle / truncated prismatoid but instead a general convex cell. 



%The volume of the intersection with the neighbour cell can then be approximated as the volume of the truncated prismatoid (or two truncated prismatoids in case the polygons intersect) defined by the two polygons. Figure \ref{fig:voronoi_cases_3D} illustrates these possible cases. 

This approximation is central to the performance of our algorithm, but it comes with the following concessions to accuracy:
\begin{enumerate}
    \item If the face of a neighbour with the merged cell has less vertices than the face with the original cell, the truncated prismatoid will slightly underestimate the volume of the true intersection. See Figure \ref{fig:Prismatoid} for an example.

    \item The approximation assumes that the triangulation after the edge collapse is still Delaunay. However, edges of the merged cell may no longer be valid and new edges between neighbour cells may be enabled by removing the original two points. In a 2D Delaunay triangulation, each such instance would lead to an edge flip. One such example is visualized in Figure \ref{fig:edgeflips}. In a 3D triangulation, this causes a bistellar flip, creating new edges between neighbours of $V_i$ and $V_j$ and causing other neighbours to not share a connection with $\hat{V}_{new}$. The newly introduced Delaunay edges create a new face between the two neighbours, which is not considered by the set of halfplanes $\mathcal{H}$ used to compute the volume of the intersection.
    
    
    \item If the neighbour does not share a face with the merged cell, we approximate it as a pyramid with the original face $\mathcal{F}_{orig}$ as the base and the apex at $\mathbf{c} + height \cdot \textsc{normal}(\mathcal{F}_{orig})$. 

    
\end{enumerate}





\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[angle=90,origin=c,width=0.6\linewidth]{Figures/CellMerge.png}
        \caption{Cell Merge}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{Figures/Cases_3D/Prismatoid.png}
        \caption{Case 1: Truncated Prismatoid}
    \end{subfigure}\\
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{Figures/Cases_3D/DoubleWedge.png}
        \caption{Case 2: Double Wedge / 2 truncated prismatoids}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        %\includegraphics[angle=180,origin=c,width=0.6\linewidth]{Figures/Cases_3D/Pyramid.png}
        %\caption{Case 3: Pyramid}
    \end{subfigure}

    \caption{The intersection volume is approximated either as a truncated prismatoid or double wedge shape between $\mathcal{F}_{orig}$ (blue) and $\mathcal{F}_{new}$ (red).}
    \label{fig:voronoi_cases_3D}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{Figures/Cases_3D/ApproxPyramid.png}
        \caption{Case 3: Convex cell (blue) approximated as Pyramid (red).}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{Figures/Cases_3D/ApproxTruncatedPrismatoid.png}
        \caption{Case 4: Convex cell (blue) approximated as truncated Prismatoid (red).}
    \end{subfigure}
    \hspace{2mm}
    \caption{ Approximations used to parallelize intersection volume calculations.}
    \label{fig:Prismatoid}
\end{figure}


\begin{algorithm}
\caption{Compute Cost}
\label{alg:voronoi_prismatoid_signed}
\begin{algorithmic}[1]

\Function{ComputeCost}{$(i, j) \in \mathcal{T}_\mathcal{E}$}

\State $\mathbf{x}_{new} \gets \frac{\mathbf{x}_i + \mathbf{x}_j}{2} $\Comment{Midpoint}
\State $\mathbf{y}_{new} \gets \text{\textsc{InterpolateValue}}(\mathbf{y}_i, \mathbf{y}_j)$

\State{$cost \gets 0$}
\For{$k \in \{i, j\}$}
    \State{$\hat{V} \gets \text{\textsc{Volume}}(V_k)$}
    \For{$n \in \mathcal{N}(k)$} 
        \State $\mathcal{H} \gets \{\textsc{PerpBisector}(n,o) |o \in \big( \mathcal{N}(n) \cap \mathcal{N}(k) \big)\}$
        \State $\Pi_{new} \gets \text{\textsc{PerpBisector}}(\mathbf{x}_n, \mathbf{x}_{new})$
        \State $\Pi_{\text{orig}} \gets \text{\textsc{PerpBisector}}(\mathbf{x}_n, \mathbf{x}_k)$

        \State $\mathcal{F}_{\text{orig}} \gets \Pi_{orig} \cap{\mathcal{H}}$
        
        \State $\mathcal{F}_{new} \gets \Pi_{new} \cap{\mathcal{H}}$
        \If{$\mathcal{F}_{new} \cap \mathcal{F}_{orig} == \emptyset$}\Comment{Prismatoid Case}
        \If{$\mathcal{F}_{new} \cap \mathcal{H} ==\emptyset $}
            \Comment{Cone-like case}
            \State{$\mathbf{c} \gets \frac{\text{vertices}(\mathcal{F}_{\text{orig}})}{|\text{vertices}(\mathcal{F}_{\text{orig}})|} $}
            
            \State{$h \gets \min_t\{\mathbf{c} + t\cdot \textsc{Normal}(\mathcal{F}_{\text{orig}}) \in \mathcal{H})$}
            \State{}\Comment{Top Polygon becomes Point}
            \State{$F_M \gets \mathbf{c} + h\cdot \textsc{Normal}(\mathcal{F}_{\text{orig}})$} 
        \EndIf
        \State{$V_{k,N} \gets \text{\textsc{BetweenVolume}}(\mathcal{F}_{new}, \mathcal{F}_{orig})$}
        \State{$cost \gets cost + V_{k,N} \cdot (\mathbf{y}_k - \mathbf{y}_n)^2$}
        \State{$\hat{V} \gets \hat{V} - V_{k,N}$}
            
        \Else
        \Comment{Double Wedge case}
            
            \State{$\Pi \gets \text{\textsc{HalfPlane}}(\mathcal{F}_{new} \cap \mathcal{F}_{orig}, \text{normal}(\mathcal{F}_{orig}))$}
            \State{}\Comment{$\Pi$ splits the polygons along the intersection}

            
            \State{$V_{k,N}^+ \gets \text{\textsc{PrismVolume}}(\mathcal{F}_M \cap\Pi, \mathcal{F}_{orig} \cap\Pi)$}
            \State{$V_{k,N}^- \gets \text{\textsc{PrismVolume}}(\mathcal{F}_M \setminus \Pi, \mathcal{F}_{orig} \setminus \Pi)$}



            \State{$cost \gets cost + (V_{k,N}^+ + V_{k,N}^-) \cdot (\mathbf{y}_k - \mathbf{y}_n)^2$}
            \State{$\hat{V} \gets \hat{V} - V_{k,N}^-+V_{k,N}^+$}
        \EndIf
        
    \EndFor
    \State{$cost \gets cost + \hat{V} \cdot (\mathbf{y}_k - \mathbf{y}_{new})^2$}
\EndFor
\State \Return $cost$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> Sections/Claude_Only.tex <==
% =====================================================================
%  Section 4.2.1.1 -- Neighbour Intersection Volumes (draft)
%
%  Requires: amsmath, amssymb, amsthm (lemma/proposition/theorem/
%  definition/corollary/remark environments), xcolor, booktabs,
%  algorithm + algpseudocode.
%
%  Labels assumed from the rest of the paper (adjust as needed):
%    eq:cost_i    -> Eq. (15)   gained volume of neighbours of i
%    eq:cost_j    -> Eq. (16)   gained volume of neighbours of j
%    eq:cost_new  -> Eq. (17)   volume lost by neighbours to V_new
%    eq:locality  -> Eq. (14)
%    eq:face      -> Eq. (8)
%    prop:inherit -> Proposition 1 (Eq. 22)
%    alg:prism    -> Algorithm 3
% =====================================================================
 
\providecommand{\figidea}[1]{\par\noindent\textcolor{blue}{\textbf{[Figure idea]} #1}\par}
\providecommand{\TODO}[1]{\textcolor{red}{\textbf{TODO}: #1}}
\providecommand{\Vol}{\operatorname{Vol}}
\providecommand{\conv}{\operatorname{conv}}
 
\paragraph{Approximating Neighbour Intersection Volumes}
\label{sec:neighbour_volumes}
 
Throughout this section, the sites $\mathbf{x}_i$ and $\mathbf{x}_j$ are merged
into $\mathbf{x}_{new} = \frac{1}{2}(\mathbf{x}_i + \mathbf{x}_j)$, and quantities
after the merge are marked with a hat: $\hat V_k$, $\hat{\mathcal{N}}(k)$,
$\hat{\mathcal{F}}_{k,l}$ and $\hat{\mathcal{T}}$. We assume the sites are in
general position, i.e.\ no four sites are coplanar and no five are cospherical.
In particular, two Voronoi cells intersect if and only if their sites share a
Delaunay edge. Recall that $\Pi^+_{\mathbf{a},\mathbf{b}}$ denotes the closed
half-space of points at least as close to $\mathbf{a}$ as to $\mathbf{b}$.
 
For a neighbour $k$ of $i$, the cost terms in Equations~\ref{eq:cost_i} and
\ref{eq:cost_new} require two volumes:
\begin{align}
  G_k &:= V_i \cap \hat V_k      && \text{(volume $k$ gains from $V_i$)},\\
  L_k &:= V_k \cap \hat V_{new}  && \text{(volume $k$ loses to $\hat V_{new}$)}.
\end{align}
We first treat neighbours of only one merged cell, $k\in\mathcal{N}(i)\setminus\mathcal{N}(j)$.
Neighbours of both cells are reduced to this case at the end of the section.
 
\subparagraph{Two locality lemmas.}
We begin with two observations that confine the effect of a merge.
 
\begin{lemma}[The shared face is absorbed]
\label{lem:absorb}
$\mathcal{F}_{i,j} \subset \operatorname{int} \hat V_{new}$.
\end{lemma}
\begin{proof}
For any point $\mathbf{p}$, expanding $\|\mathbf{p}-\mathbf{x}_{new}\|^2$ gives
\begin{equation}
  \|\mathbf{p}-\mathbf{x}_{new}\|^2
  = \tfrac{1}{2}\|\mathbf{p}-\mathbf{x}_i\|^2 + \tfrac{1}{2}\|\mathbf{p}-\mathbf{x}_j\|^2
    - \tfrac{1}{4}\|\mathbf{x}_i-\mathbf{x}_j\|^2 .
  \label{eq:midpoint_identity}
\end{equation}
For $\mathbf{p}\in\mathcal{F}_{i,j}$ we have
$\|\mathbf{p}-\mathbf{x}_i\| = \|\mathbf{p}-\mathbf{x}_j\| =: r$. Hence
$\|\mathbf{p}-\mathbf{x}_{new}\|^2 = r^2 - \tfrac14\|\mathbf{x}_i-\mathbf{x}_j\|^2 < r^2$.
Every remaining site $\mathbf{x}_l$ satisfies $\|\mathbf{p}-\mathbf{x}_l\| \ge r$.
\end{proof}
 
Lemma~\ref{lem:absorb} holds for any $\mathbf{x}_{new}$ on the open segment
between $\mathbf{x}_i$ and $\mathbf{x}_j$, not only the midpoint.
 
\begin{lemma}[Cells only gain from neighbours]
\label{lem:locality}
Let $k \notin \{i,j\}$. If $\hat V_k \cap V_j \neq \emptyset$, then $k\in\mathcal{N}(j)$.
The same holds with $i$ in place of $j$.
\end{lemma}
\begin{proof}
Let $\mathbf{p}\in\hat V_k$. Every old site other than $i$ and $j$ is at least
as far from $\mathbf{p}$ as $\mathbf{x}_k$. Hence
$\hat V_k \subseteq V_k \cup V_i \cup V_j$.
 
Suppose $\mathbf{p}\in\hat V_k\cap V_j$, and consider the segment $[\mathbf{x}_k,\mathbf{p}]$.
It lies in $\hat V_k$ by convexity, so it is covered by the two closed sets
$V_k\cup V_i$ and $V_j$. Both contain a point of the segment, and the segment is
connected. Therefore the segment contains a point $\mathbf{z}$ in both sets.
 
If $\mathbf{z} \in V_i\cap V_j=\mathcal{F}_{i,j}$, then
$\mathbf{z}\in\operatorname{int}\hat V_{new}$ by Lemma~\ref{lem:absorb}. This
contradicts $\mathbf{z}\in\hat V_k$. Hence $\mathbf{z}\in V_k\cap V_j$, which by
general position implies $k\in\mathcal{N}(j)$.
\end{proof}
 
Lemma~\ref{lem:locality} shows that the sums over $\mathcal{N}(i)$ and $\mathcal{N}(j)$
in Equations~\ref{eq:cost_i} and \ref{eq:cost_j} are complete. For
$k \in \mathcal{N}(i)\setminus\mathcal{N}(j)$, it also gives
\begin{equation}
  G_k = \hat V_k \cap \Pi^+_{\mathbf{x}_i,\mathbf{x}_k}.
  \label{eq:gain_region}
\end{equation}
To see this, take a point of $\hat V_k$ that is at least as close to
$\mathbf{x}_i$ as to $\mathbf{x}_k$. Its old nearest site is $i$ or $j$, and
Lemma~\ref{lem:locality} excludes $j$.
 
\TODO{Eq.~\ref{eq:cost_new} sums over $\mathcal{N}(i)\cup\mathcal{N}(j)$.
If $(i,j)$ is not a Gabriel edge, $\mathbf{x}_{new}$ lies inside the cell of a
third site. $\hat V_{new}$ may then take volume from cells that neighbour
neither $i$ nor $j$. Verify empirically or prove that this cannot happen.}
 
\subparagraph{Neighbour tunnel and faces.}
We call
\begin{align}
  \mathcal{H}_{k,i} &:= \{\Pi^+_{\mathbf{x}_k,\mathbf{x}_l} \mid l\in\mathcal{N}(k)\cap\mathcal{N}(i)\},\\
  \mathcal{C}_{k,i} &:= \textstyle\bigcap \mathcal{H}_{k,i}
\end{align}
the \emph{neighbour tunnel} of $k$ towards $i$. Every half-space in
$\mathcal{H}_{k,i}$ remains a constraint of $\hat V_k$ after the merge,
since $j\notin\mathcal{N}(k)$ and all other common neighbours remain sites.
Hence
\begin{equation}
  \hat V_k\subseteq\mathcal{C}_{k,i}.
  \label{eq:tunnel_contains}
\end{equation}
For a face $\mathcal{F}$ of $V_k$ or $\hat V_k$, we denote by
\begin{equation}
  \mathcal{E}(\mathcal{F}) := \{\,l \mid \mathcal{F}\cap\Pi_{\mathbf{x}_k,\mathbf{x}_l}
  \text{ is an edge of }\mathcal{F}\}
\end{equation}
the sites whose wall supports an edge of $\mathcal{F}$. We have
$\mathcal{E}(\mathcal{F}_{k,i})\subseteq\mathcal{N}(k)\cap\mathcal{N}(i)$.
The walls of the remaining common neighbours are redundant on
$\mathcal{F}_{k,i}$ (cf.\ Equation~\ref{eq:face}), but they may become active
between the old and the new face. The original and new faces are
\begin{equation}
  \mathcal{F}_{orig} := \Pi_{\mathbf{x}_k,\mathbf{x}_i}\cap\mathcal{C}_{k,i},
  \qquad
  \mathcal{F}_{new}  := \Pi_{\mathbf{x}_k,\mathbf{x}_{new}}\cap\mathcal{C}_{k,i}.
  \label{eq:tunnel_faces}
\end{equation}
A convex polygon is the intersection of the half-planes supporting its edges.
Hence $\mathcal{F}_{orig}=\mathcal{F}_{k,i}$ exactly. Whether
$\mathcal{F}_{new}$ equals the true face $\hat{\mathcal{F}}_{k,new}$ depends on
the changes to the triangulation, as discussed below.
 
\figidea{3D rendering of a cell $V_k$ with the face $\mathcal{F}_{orig}$
highlighted and the tunnel walls $\Pi_{\mathbf{x}_k,\mathbf{x}_l}$,
$l\in\mathcal{N}(k)\cap\mathcal{N}(i)$, extended as translucent planes towards $\mathbf{x}_i$.
The tilted plane $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$ cuts the tunnel in
$\mathcal{F}_{new}$, and the region between the two faces is shaded.}
 
\subparagraph{Truncated prismatoids.}
The regions we compute are all of the following shape.
 
\begin{definition}[Truncated prismatoid]
A \emph{truncated prismatoid} is a convex polyhedron $P$ whose vertices all lie
in the union of two planes $E_1, E_2$, with $P = \conv\big((P\cap E_1)\cup(P\cap E_2)\big)$.
The two \emph{bases} $P\cap E_1$ and $P\cap E_2$ are convex polygons and may
degenerate to a segment or a point.
\end{definition}
 
Unlike a classical prismatoid, the planes need not be parallel. The definition
includes wedges, whose two bases share an edge, and pyramids, where one base is
a point. The volume of a truncated prismatoid follows from a tetrahedral
decomposition (Algorithm~\ref{alg:prism}). The number of tetrahedra is linear
in the number of base vertices, and there is no data-dependent branching.
 
\subparagraph{The side of the shared face.}
The face $\mathcal{F}_{new}$ may lie on either side of $\mathcal{F}_{orig}$, or
the two faces may cross. Define the affine function
\begin{equation}
  \sigma_i(\mathbf{p}) := \|\mathbf{p}-\mathbf{x}_{new}\|^2 - \|\mathbf{p}-\mathbf{x}_i\|^2 .
\end{equation}
Its zero set is the bisector $\Pi_{\mathbf{x}_i,\mathbf{x}_{new}}$. By
Equation~\ref{eq:midpoint_identity}, this plane is parallel to
$\Pi_{\mathbf{x}_i,\mathbf{x}_j}$, halfway between $\mathbf{x}_i$ and
$\Pi_{\mathbf{x}_i,\mathbf{x}_j}$. For a polygon $\mathcal{F}$, let
$\mathcal{F}^{\pm} := \mathcal{F}\cap\{\pm\sigma_i\ge 0\}$.
 
\begin{lemma}[Separation of gain and loss]
\label{lem:separation}
$G_k \subseteq \{\sigma_i \ge 0\}$ and $L_k \subseteq \{\sigma_i\le 0\}$.
\end{lemma}
\begin{proof}
For $\mathbf{p}\in G_k$ we have
$\|\mathbf{p}-\mathbf{x}_i\|\le\|\mathbf{p}-\mathbf{x}_k\|\le\|\mathbf{p}-\mathbf{x}_{new}\|$.
For $\mathbf{p}\in L_k$ we have
$\|\mathbf{p}-\mathbf{x}_{new}\|\le\|\mathbf{p}-\mathbf{x}_k\|\le\|\mathbf{p}-\mathbf{x}_i\|$.
\end{proof}
 
On $\Pi_{\mathbf{x}_k,\mathbf{x}_i}$ and on $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$,
the two faces can only meet on the line
$\Pi_{\mathbf{x}_k,\mathbf{x}_i}\cap\Pi_{\mathbf{x}_i,\mathbf{x}_{new}}$.
Hence the plane $\Pi_{\mathbf{x}_i,\mathbf{x}_{new}}$ splits both faces
consistently into a gained part and a lost part.
 
\subsubsection*{The flip-free case}
 
We first consider merges that change the Delaunay tetrahedralisation only
through the collapse of the edge $(i,j)$. Formally, let
$\hat{\mathcal{T}} = \mathcal{T}/(i,j)$ be the contraction of $\mathcal{T}$
along $(i,j)$: tetrahedra containing both $i$ and $j$ are removed, and $i$ and
$j$ are identified with $new$ in all remaining tetrahedra.
 
\begin{theorem}[Exactness without flips]
\label{thm:noflip}
Let $k\in\mathcal{N}(i)\setminus\mathcal{N}(j)$ and $\hat{\mathcal{T}} = \mathcal{T}/(i,j)$. Then
\begin{enumerate}
  \item $\mathcal{F}_{new} = \hat{\mathcal{F}}_{k,new}$;
  \item $G_k = \conv\!\big(\mathcal{F}^+_{orig}\cup\mathcal{F}^+_{new}\big)$ and
        $L_k = \conv\!\big(\mathcal{F}^-_{orig}\cup\mathcal{F}^-_{new}\big)$.
        Both are truncated prismatoids.
\end{enumerate}
In particular, if $\sigma_i$ has a constant sign on $\mathcal{F}_{orig}$, one of
the two regions is empty. Otherwise the two faces cross and $k$ both gains and
loses volume, which we call a \emph{double wedge}.
\end{theorem}
 
\begin{proof}
\emph{(1)} Under contraction, $\hat{\mathcal{N}}(k) = (\mathcal{N}(k)\setminus\{i\})\cup\{new\}$,
so $\hat V_k$ is $V_k$ with $\Pi^+_{\mathbf{x}_k,\mathbf{x}_i}$ replaced by
$\Pi^+_{\mathbf{x}_k,\mathbf{x}_{new}}$. The edges of a Voronoi face correspond
to the Delaunay triangles containing its dual edge. The contraction maps the
triangles $\{k,i,l\}$ to $\{k,new,l\}$, hence
$\mathcal{E}(\hat{\mathcal{F}}_{k,new})=\mathcal{E}(\mathcal{F}_{k,i})\subseteq\mathcal{N}(k)\cap\mathcal{N}(i)$.
By Equation~\ref{eq:tunnel_contains},
$\hat{\mathcal{F}}_{k,new}=\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}\cap\hat V_k\subseteq\mathcal{F}_{new}$.
Conversely, $\mathcal{F}_{new}$ satisfies all constraints of
$\mathcal{E}(\hat{\mathcal{F}}_{k,new})$. A convex polygon is the intersection
of its edge half-planes, so $\mathcal{F}_{new}\subseteq\hat{\mathcal{F}}_{k,new}$.
 
\emph{(2), gained part.} By Equation~\ref{eq:gain_region},
$G_k = \Pi^+_{\mathbf{x}_i,\mathbf{x}_k}\cap\Pi^+_{\mathbf{x}_k,\mathbf{x}_{new}}
\cap\bigcap_{l\in\mathcal{N}(k)\setminus\{i\}}\Pi^+_{\mathbf{x}_k,\mathbf{x}_l}$.
Consider a vertex $\mathbf{v}$ of $G_k$ that lies on neither
$\Pi_{\mathbf{x}_k,\mathbf{x}_i}$ nor $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$. It
lies on three walls $\Pi_{\mathbf{x}_k,\mathbf{x}_{l_1}},\Pi_{\mathbf{x}_k,\mathbf{x}_{l_2}},\Pi_{\mathbf{x}_k,\mathbf{x}_{l_3}}$,
so it is the circumcentre of a tetrahedron $\{k,l_1,l_2,l_3\}\in\hat{\mathcal{T}}$.
Since $\mathbf{v}$ is strictly closer to $\mathbf{x}_i$ than to $\mathbf{x}_k$,
this tetrahedron is not in $\mathcal{T}$. It is not incident to $i$ or $j$, so
it is not in $\mathcal{T}/(i,j)$ either, which is a contradiction.
 
Hence all vertices of $G_k$ lie on the two planes. On
$\Pi_{\mathbf{x}_k,\mathbf{x}_i}$, the constraint
$\Pi^+_{\mathbf{x}_k,\mathbf{x}_{new}}$ is equivalent to $\sigma_i\ge 0$. On
$\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$, the constraint
$\Pi^+_{\mathbf{x}_i,\mathbf{x}_k}$ is also equivalent to $\sigma_i\ge 0$.
Therefore the two bases are $\mathcal{F}^+_{orig}$ and $\mathcal{F}^+_{new}$.
 
\emph{(2), lost part.} Every point of $V_k$ that is closer to $\mathbf{x}_{new}$
than to $\mathbf{x}_k$ is closer to $\mathbf{x}_{new}$ than to any site.
Hence, in general,
\begin{equation}
  L_k = V_k\cap\Pi^+_{\mathbf{x}_{new},\mathbf{x}_k}.
  \label{eq:loss_region}
\end{equation}
Consider a vertex of $L_k$ on neither plane. It is a Voronoi vertex of $V_k$,
i.e.\ the circumcentre of a tetrahedron $\{k,l_1,l_2,l_3\}\in\mathcal{T}$ that
is not incident to $i$ or $j$. This circumcentre is strictly closer to
$\mathbf{x}_{new}$ than to the tetrahedron's vertices, so the tetrahedron is
not in $\hat{\mathcal{T}}$. This contradicts
$\hat{\mathcal{T}}=\mathcal{T}/(i,j)$. The identification of the bases follows
as for the gained part.
\end{proof}
 
In the flip-free case, the vertices of $\mathcal{F}_{orig}$ and
$\mathcal{F}_{new}$ correspond one-to-one along the Voronoi edges
$\Pi_{\mathbf{x}_k,\mathbf{x}_{l}}\cap\Pi_{\mathbf{x}_k,\mathbf{x}_{l'}}$.
All lateral faces are therefore planar quadrilaterals, and pairing vertices by
index in Algorithm~\ref{alg:prism} is exact. In the double wedge, the two
crossing points are shared by both bases.
 
\TODO{When the vertex counts differ (flip cases below), check that the
index-based pairing with padded duplicates in Algorithm~\ref{alg:prism}
reproduces the lateral faces of the convex hull.}
 
The sign test replaces the polygon intersection test
$\mathcal{F}_{M}\cap\mathcal{F}_{orig}=\emptyset$ of the original cost
algorithm. We evaluate the affine function $\sigma_i$ at the vertices of both
faces and clip both faces with the single plane
$\Pi_{\mathbf{x}_i,\mathbf{x}_{new}}$.
 
\figidea{2D cross-section of the double wedge. A concrete configuration is
$\mathbf{x}_i=(0,0)$, $\mathbf{x}_j=(4,0)$, $\mathbf{x}_k=(0,2)$ and a blocking
site $\mathbf{x}_l=(3,2)$, so that $k\notin\mathcal{N}(j)$. The old face lies
on $y=1$ and the new face on $y=x$. They cross at $(1,1)$ on the line $x=1$,
which is $\Pi_{\mathbf{x}_i,\mathbf{x}_{new}}$. Colour the gained region (left)
and the lost region (right) separately, and draw the plane $x=1$ dashed.
This also shows that crossing faces occur even for Gabriel edges and without
any flip.}
 
\subsubsection*{Merges with flips}
 
In general, the merge also changes Delaunay simplices around $\mathbf{x}_k$
beyond the contraction. The polytope $G_k$ is then bounded by
$\Pi_{\mathbf{x}_k,\mathbf{x}_i}$, possibly by $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$,
and by a set of walls that may differ from $\mathcal{H}_{k,i}$. We distinguish
three situations, which may occur simultaneously. Our algorithm treats all of
them uniformly: it always evaluates Equation~\ref{eq:tunnel_faces} and falls
back to a separate approximation only in Case~3.
 
\paragraph{Case 1: Vertex loss.}
In this case every wall bounding $G_k$ belongs to $\mathcal{H}_{k,i}$, but two
walls may meet before reaching $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$. The
lateral face on $\Pi_{\mathbf{x}_k,\mathbf{x}_l}$ then pinches out at a vertex
$\mathbf{v}$ strictly between the two planes, and $\mathcal{F}_{new}$ loses the
edge on that wall. The tunnel face is still exact on the
gained side, because $\hat V_k$ is cut by the same walls:
$\mathcal{F}^+_{new} = \hat{\mathcal{F}}^+_{k,new}$. However, $G_k$ now has the
additional vertex $\mathbf{v}$, so $G_k$ is no longer a truncated prismatoid.
 
We keep only the two faces and approximate $G_k$ by
$\conv(\mathcal{F}^+_{orig}\cup\mathcal{F}^+_{new})$. Since $G_k$ is convex and
contains both faces, this \emph{underestimates} $\Vol(G_k)$. The missing volume
lies in small caps around the pinch vertices. Importantly, vertex loss does not
change which cells are neighbours:
 
\begin{proposition}[Vertex loss preserves neighbourhoods]
\label{prop:vertex_loss}
Assume every wall bounding $G_k$ belongs to $\mathcal{H}_{k,i}$, and let $l$ be
the site of a pinched lateral face with adjacent walls $l_1, l_2$. Then:
\begin{enumerate}
  \item every $l'$ whose wall supports an edge of
        $\mathcal{F}^+_{orig}$ remains a neighbour of $k$; in particular,
        $l\in\hat{\mathcal{N}}(k)$;
  \item every $l'\in\mathcal{E}(\hat{\mathcal{F}}_{k,new})$ is a neighbour of $new$; in
        particular, $l_1,l_2\in\hat{\mathcal{N}}(new)$;
  \item the triangle $\{k,new,l\}$ is not in $\hat{\mathcal{T}}$, while the
        tetrahedron $\{k,l_1,l,l_2\}$ is.
\end{enumerate}
\end{proposition}
\begin{proof}
\emph{(1)} Let $l'$ be such a site. The wall $\Pi_{\mathbf{x}_k,\mathbf{x}_{l'}}$
supports an edge of $\mathcal{F}^+_{orig}$ of positive length. Because the
pinch vertices lie strictly between the two planes, $G_k$ has a facet of
positive area on this wall. Every point of that facet is equidistant from
$\mathbf{x}_k$ and $\mathbf{x}_{l'}$ and nearest to both. Hence the facet lies
in $\hat{\mathcal{F}}_{k,l'}$.
 
\emph{(2)} Each $l'\in\mathcal{E}(\hat{\mathcal{F}}_{k,new})$ supports an edge
of $\hat{\mathcal{F}}_{k,new}$. This edge is dual to the triangle
$\{k,new,l'\}\in\hat{\mathcal{T}}$, which contains the edge $(new,l')$.
 
\emph{(3)} The pinch vertex $\mathbf{v}$ is equidistant from
$\mathbf{x}_k,\mathbf{x}_{l_1},\mathbf{x}_l,\mathbf{x}_{l_2}$ and lies in
$\hat V_k$. It is therefore the circumcentre of a Delaunay tetrahedron of
$\hat{\mathcal{T}}$. The lateral face of $l$ ends at $\mathbf{v}$ and does not
reach $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$. Hence $l\notin\mathcal{E}(\hat{\mathcal{F}}_{k,new})$,
i.e.\ the triangle $\{k,new,l\}$ is not in $\hat{\mathcal{T}}$.
\end{proof}
 
In the simplest instance, this is a $2\!\to\!3$ bistellar flip. The two
tetrahedra $\{k,new,l_1,l\}$ and $\{k,new,l,l_2\}$ of $\mathcal{T}/(i,j)$ are
replaced by $\{k,new,l_1,l_2\}$, $\{new,l,l_1,l_2\}$ and $\{k,l_1,l,l_2\}$. This
creates the edge $(l_1,l_2)$ but removes no edge incident to $k$ or $new$.
 
Such a flip has no counterpart in 2D. There, Voronoi faces are segments with
exactly two vertices, and by planarity every flip adds or removes an edge
incident to the merged site.
 
Proposition~\ref{prop:vertex_loss} concerns the gained side. On the lost side,
a vertex loss of $\mathcal{F}^-_{new}$ means that $\hat V_{new}$ swallows a
Voronoi vertex of $V_k$. This can remove a neighbour of $k$ entirely, since the
region is given exactly by Equation~\ref{eq:loss_region}.
 
\figidea{Pinching in 3D: the tunnel between $\mathcal{F}_{orig}$ (blue) and
$\mathcal{F}_{new}$ (red). One lateral face is a triangle ending at the pinch
vertex $\mathbf{v}$. Include an inset with the corresponding $2\!\to\!3$ flip,
showing the tetrahedra before and after and the new edge $(l_1,l_2)$.}
 
\paragraph{Case 2: New walls.}
In this case $G_k$ is bounded by a wall $\Pi_{\mathbf{x}_k,\mathbf{x}_l}$ that
is not in the tunnel, i.e.\ $l\notin\mathcal{N}(k)\cap\mathcal{N}(i)$. Such a
site becomes a new neighbour of $k$ through a flip. Walls of common neighbours
that are redundant on $\mathcal{F}_{orig}$ but become active between the faces
are already contained in $\mathcal{H}_{k,i}$. New walls cannot come from
arbitrary cells:
 
\begin{proposition}[New walls come from $\mathcal{N}(i)$]
\label{prop:new_walls}
If $G_k$ has a facet on $\Pi_{\mathbf{x}_k,\mathbf{x}_l}$ with $l\ne new$, then
$l\in\mathcal{N}(i)$. Consequently,
\begin{equation}
  G_k = V_i\cap\Pi^+_{\mathbf{x}_k,\mathbf{x}_{new}}\cap
        \bigcap_{l\in\mathcal{N}(i)\setminus\{j,k\}}\Pi^+_{\mathbf{x}_k,\mathbf{x}_l}.
  \label{eq:exact_gain}
\end{equation}
\end{proposition}
\begin{proof}
The facet lies in $V_i$ and borders $\hat V_l$, so
$\hat V_l\cap V_i\ne\emptyset$. By Lemma~\ref{lem:locality}, $l\in\mathcal{N}(i)$.
 
For Equation~\ref{eq:exact_gain}, the inclusion $\subseteq$ is immediate. For
$\supseteq$, let $\mathbf{p}$ lie in the right-hand side and let $t$ be its
nearest new site. The constraint $\Pi^+_{\mathbf{x}_k,\mathbf{x}_{new}}$ allows
us to take $t\ne new$. Then $\mathbf{p}\in\hat V_t\cap V_i$, so
$t\in\mathcal{N}(i)$ by Lemma~\ref{lem:locality}. The constraint
$\Pi^+_{\mathbf{x}_k,\mathbf{x}_t}$ then gives $\mathbf{p}\in\hat V_k$.
\end{proof}
 
Proposition~\ref{prop:new_walls} shows that the exact gained region never
requires a local reconstruction of the triangulation. It is an intersection of
roughly $|\mathcal{N}(i)|\approx 16$ known half-spaces. However, computing its
volume means clipping a general convex polytope, with a data-dependent number
of active planes and vertices. This causes divergent control flow and memory
access on the GPU.
 
As an engineering choice, we therefore ignore the walls of new neighbours
$l\in\mathcal{N}(i)\setminus\mathcal{N}(k)$. We compute $\mathcal{F}_{new}$
from the tunnel alone, as if the neighbourhood of $k$ were unchanged. The tunnel region then contains $G_k$, and the tunnel
face contains the true face, so this approximation tends to
\emph{overestimate} the gained volume. Cases~1 and~2 can occur for the same
neighbour, with opposite biases, so the sign of the combined error is not
determined.
 
Note that pruning the tunnel to $\mathcal{E}(\mathcal{F}_{k,i})$, i.e.\ to
the walls that are active on the old face, is not lossless. Walls of common
neighbours that are redundant on $\mathcal{F}_{orig}$ can become active between
the faces, and pruning would move them into Case~2.
 
\figidea{Case 2: the same tunnel as in the Case 1 figure, with an additional
wall $\Pi_{\mathbf{x}_k,\mathbf{x}_l}$, $l\in\mathcal{N}(i)\setminus\mathcal{N}(k)$,
cutting a corner off the region between the faces. Shade the overestimated
volume.}
 
\paragraph{Case 3: Tunnel closure.}
In this case the tunnel closes on the gained side before reaching
$\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$, so $\mathcal{F}^+_{orig}\ne\emptyset$
but $\mathcal{F}^+_{new}=\emptyset$. In the most common instance, $k$ and $new$
are no longer Delaunay neighbours: $k$ does not inherit its edge to $i$.
 
\begin{proposition}[Tunnel closure]
\label{prop:closure}
\begin{enumerate}
  \item $\hat{\mathcal{F}}^+_{k,new}\subseteq\mathcal{F}^+_{new}$. Hence, if
        the tunnel closes, $G_k$ shares no facet with $\hat V_{new}$.
  \item If $(k,new)\notin\hat{\mathcal{T}}_\mathcal{E}$, then $L_k=\emptyset$,
        and only the gained volume contributes to the cost.
\end{enumerate}
\end{proposition}
\begin{proof}
\emph{(1)} This follows from $\hat V_k\subseteq\mathcal{C}_{k,i}$
(Equation~\ref{eq:tunnel_contains}).
 
\emph{(2)} Suppose $L_k = V_k\cap\Pi^+_{\mathbf{x}_{new},\mathbf{x}_k}$ has
positive volume. Since $\mathbf{x}_k\in\operatorname{int}V_k\setminus L_k$, the
plane $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$ cuts the interior of $V_k$. The
resulting cross-section has positive area and consists of points nearest to
both $\mathbf{x}_k$ and $\mathbf{x}_{new}$. It therefore lies in
$\hat{\mathcal{F}}_{k,new}$, so $(k,new)\in\hat{\mathcal{T}}_\mathcal{E}$.
\end{proof}
 
We approximate the closed region by a pyramid over $\mathcal{F}^+_{orig}$. Let
$\mathbf{c}$ be the vertex centroid of $\mathcal{F}^+_{orig}$, and let
$\mathbf{n} = (\mathbf{x}_i-\mathbf{x}_k)/\|\mathbf{x}_i-\mathbf{x}_k\|$ be its
normal pointing into $V_i$. The apex is placed at $\mathbf{c}+h\,\mathbf{n}$,
where $h$ is the distance at which the ray first leaves the tunnel:
\begin{equation}
  h = \min_{\substack{l\in\mathcal{N}(k)\cap\mathcal{N}(i)\\ \mathbf{n}\cdot(\mathbf{x}_l-\mathbf{x}_k)>0}}
      \frac{\big(\tfrac12(\mathbf{x}_k+\mathbf{x}_l)-\mathbf{c}\big)\cdot(\mathbf{x}_l-\mathbf{x}_k)}
           {\mathbf{n}\cdot(\mathbf{x}_l-\mathbf{x}_k)} .
\end{equation}
The ray is orthogonal to the base, so
$\Vol = \tfrac13\,\operatorname{Area}(\mathcal{F}^+_{orig})\,h$ and no
triangulation of the lateral surface is required. The pyramid may over- or
underestimate $\Vol(G_k)$.
 
The test is conservative. By Proposition~\ref{prop:closure}, closure of the
tunnel implies closure of the true region on the gained side. The converse does
not hold: if the true region closes only because of a wall outside
$\mathcal{H}_{k,i}$, the tunnel face is non-empty and the neighbour is handled
as in Cases~1 and~2.
 
\figidea{Case 3: the tunnel converging to a tip before reaching
$\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$, with the approximating pyramid (red)
overlaid on the true convex cell (blue). This extends Figure~9a with the ray
from $\mathbf{c}$ along $\mathbf{n}$ and the wall it hits first.}
 
\subsubsection*{Neighbours of both merged cells}
 
If $k\in\mathcal{N}(i)\cap\mathcal{N}(j)$, we split the gained region along
$\Pi_{\mathbf{x}_i,\mathbf{x}_j}$ into $\hat V_k\cap V_i$ and
$\hat V_k\cap V_j$. We treat each part with the construction above, applied to
the pairs $(k,i)$ and $(k,j)$ respectively. The wall
$\Pi^+_{\mathbf{x}_k,\mathbf{x}_j}$ of the site $j$, which no longer exists
after the merge, is replaced by $\Pi^+_{\mathbf{x}_i,\mathbf{x}_j}$ in
$\mathcal{H}_{k,i}$, and analogously for $\mathcal{H}_{k,j}$. By
Lemma~\ref{lem:absorb}, the two parts are separated by the interior of
$\hat V_{new}$, so no volume is counted twice. The lost region $L_k$ is split
along the same plane, and both parts are weighted with
$(\hat{\mathbf{y}}_{new}-\mathbf{y}_k)^2$.
 
\TODO{Extend Theorem~\ref{thm:noflip} formally to this case. The split pieces
have vertices on $\Pi_{\mathbf{x}_k,\mathbf{x}_i}$ (resp.\ $\Pi_{\mathbf{x}_k,\mathbf{x}_j}$)
and $\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}$, with one lateral face on
$\Pi_{\mathbf{x}_i,\mathbf{x}_j}$.}
 
\subsubsection*{Summary}
 
Table~\ref{tab:cases} summarises the approximations. The per-neighbour
procedure is identical in all cases except for the Case~3 fallback, so the
computation is free of data-dependent branching apart from a single test.
The resulting cost computation is given in Algorithm~\ref{alg:cost_revised}.
 
\begin{table*}[t]
\centering
\caption{Handling of neighbour intersection volumes for
$k\in\mathcal{N}(i)\setminus\mathcal{N}(j)$.}
\label{tab:cases}
\small
\begin{tabular}{@{}llll@{}}
\toprule
Configuration & Computed as & Detected & Error \\
\midrule
No flip & prismatoid(s) & -- & exact \\
Case 1: vertex loss & prismatoid, pinch vertices dropped & no & underestimate \\
Case 2: new walls & prismatoid, new walls ignored & no & overestimate \\
Case 3: tunnel closure & pyramid over $\mathcal{F}^+_{orig}$ & yes & either \\
\bottomrule
\end{tabular}
\end{table*}
 
\begin{algorithm}[t]
\caption{Compute Cost (revised)}
\label{alg:cost_revised}
\begin{algorithmic}[1]
\Function{ComputeCost}{$(i,j)\in\mathcal{T}_\mathcal{E}$}
  \State $\mathbf{x}_{new}\gets\frac12(\mathbf{x}_i+\mathbf{x}_j)$
  \State $\hat{\mathbf{y}}_{new}\gets$ \Call{InterpolateValue}{$\mathbf{y}_i,\mathbf{y}_j$}
  \State $cost\gets 0$
  \For{$m\in\{i,j\}$}
    \State $\hat V\gets\Vol(V_m)$ \Comment{Volume inherited by $\hat V_{new}$}
    \For{$k\in\mathcal{N}(m)\setminus\{i,j\}$}
      \State $\mathcal{H}\gets$ \Call{Tunnel}{$k,m$} \Comment{Walls of $\mathcal{N}(k)\cap\mathcal{N}(m)$}
      \State $\mathcal{F}_{orig}\gets\Pi_{\mathbf{x}_k,\mathbf{x}_m}\cap\mathcal{H}$
      \State $\mathcal{F}_{new}\gets\Pi_{\mathbf{x}_k,\mathbf{x}_{new}}\cap\mathcal{H}$
      \State $\mathcal{F}^\pm_{orig},\mathcal{F}^\pm_{new}\gets$ split by $\Pi_{\mathbf{x}_m,\mathbf{x}_{new}}$
      \If{$\mathcal{F}^+_{new}=\emptyset$} \Comment{Case 3}
        \State $V^+\gets$ \Call{PyramidVolume}{$\mathcal{F}^+_{orig},\mathcal{H}$}
      \Else
        \State $V^+\gets$ \Call{PrismVolume}{$\mathcal{F}^+_{orig},\mathcal{F}^+_{new}$}
      \EndIf
      \State $V^-\gets$ \Call{PrismVolume}{$\mathcal{F}^-_{orig},\mathcal{F}^-_{new}$}
      \State $cost\gets cost+V^+(\mathbf{y}_m-\mathbf{y}_k)^2+V^-(\hat{\mathbf{y}}_{new}-\mathbf{y}_k)^2$
      \State $\hat V\gets\hat V-V^+$ \Comment{Proposition~\ref{prop:inherit}}
    \EndFor
    \State $cost\gets cost+\max(\hat V,0)\,(\hat{\mathbf{y}}_{new}-\mathbf{y}_m)^2$
  \EndFor
  \State \Return $cost$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> Sections/Tables.tex <==
\begin{table*}[htbp]
\centering
\caption{Stanford Volume Scans Evaluation Benchmark ($N=250,000$ cells $\rightarrow$ $25,000$ cells, 90\% LOD Reduction). Values reported as Final MSE (Trajectory AUC Mean MSE) to 3 decimal places. Best MSE and best AUC per row are separately highlighted in \textbf{bold} (including ties up to 3 decimal places).}
\label{tab:volume_scans}
\begin{tabular}{lcccccc}
\toprule
Dataset Scene & Variance & Volume & FPS & Grid & Naive Merge  & \textbf{VoroDuce} \\
\midrule
cthead\_uniform & 0.179 (0.026) & 0.536 (0.176) & 0.418 (0.145) & 0.454 (0.187) & 0.306 (0.076) & \textbf{0.067} (\textbf{0.007}) \\
cthead\_importance & 0.501 (0.098) & 1.363 (0.270) & 0.351 (0.108) & 0.416 (0.147) & 0.440 (0.144) & \textbf{0.151} (\textbf{0.024}) \\
cthead\_gradient & 0.770 (0.197) & 1.003 (0.311) & 0.361 (0.121) & 0.439 (0.160) & 0.439 (0.151) & \textbf{0.191} (\textbf{0.052}) \\
cthead\_grid & 0.166 (0.022) & 0.663 (0.221) & 0.416 (0.157) & 0.434 (0.189) & 0.438 (0.090) & \textbf{0.128} (\textbf{0.013}) \\
mrbrain\_uniform & 0.056 (0.016) & 0.226 (0.152) & 0.175 (0.116) & 0.187 (0.083) & 0.138 (0.076) & \textbf{0.020} (\textbf{0.006}) \\
mrbrain\_importance & 0.161 (0.146) & 0.959 (0.298) & 0.160 (0.148) & 0.182 (0.067) & 0.220 (0.263) & \textbf{0.054} (\textbf{0.036}) \\
mrbrain\_gradient & 0.210 (0.115) & 0.763 (0.547) & 0.173 (0.172) & 0.193 (0.082) & 0.177 (0.166) & \textbf{0.074} (\textbf{0.047}) \\
mrbrain\_grid & 0.050 (0.020) & 0.273 (0.334) & 0.177 (0.178) & 0.172 (0.080) & 0.199 (0.155) & \textbf{0.038} (\textbf{0.016}) \\
bunny\_uniform & 0.008 (\textbf{0.001}) & 2.087 (0.652) & 1.724 (0.613) & 2.001 (0.853) & 6.706 (6.459) & \textbf{0.003} (\textbf{0.001}) \\
bunny\_importance & \textbf{0.001} (\textbf{0.000}) & 0.104 (0.013) & 0.682 (0.175) & 1.126 (0.290) & 1.055 (0.470) & \textbf{0.001} (\textbf{0.000}) \\
bunny\_gradient & 8.896 (1.884) & 2.265 (0.861) & 2.441 (0.931) & 2.668 (1.066) & 5.941 (1.743) & \textbf{1.017} (\textbf{0.217}) \\
bunny\_grid & 0.011 (0.001) & 2.916 (1.061) & 2.013 (0.902) & 2.350 (1.137) & 5.136 (4.211) & \textbf{0.003} (\textbf{0.000}) \\
\midrule
\textbf{Average} & 0.917 (0.210) & 1.096 (0.408) & 0.758 (0.314) & 0.885 (0.362) & 1.766 (1.167) & \textbf{0.146} (\textbf{0.035}) \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[htbp]
\centering
\caption{Synthetic Volumetric Data Benchmark ($N=100,000$ cells $\rightarrow$ $10,000$ cells, 90\% LOD Reduction). Values reported as Final MSE (Trajectory AUC Mean MSE) to 3 decimal places across 16 synthetic scenes.}
\label{tab:synthetic_100k}
\begin{tabular}{lcccccc}
\toprule
Dataset Scene & Variance & Volume & FPS & Grid & Naive Merge & \textbf{VoroDuce} \\
\midrule
uniform\_sine\_low & 0.082 (0.027) & 0.112 (0.028) & 0.067 (0.020) & 0.112 (0.033) & 0.074 (0.027) & \textbf{0.055} (\textbf{0.015}) \\
uniform\_sine\_high & 3.317 (1.171) & 3.319 (0.954) & 2.323 (0.743) & 3.353 (1.085) & 3.502 (1.178) & \textbf{1.906} (\textbf{0.596}) \\
uniform\_sphere & \textbf{0.000} (\textbf{0.000}) & 2.216 (0.692) & 1.534 (0.560) & 2.131 (0.721) & 3.958 (3.608) & \textbf{0.000} (\textbf{0.000}) \\
uniform\_torus & \textbf{0.000} (\textbf{0.000}) & 1.848 (0.552) & 1.227 (0.434) & 2.033 (0.547) & 8.194 (3.178) & \textbf{0.000} (\textbf{0.000}) \\
uniform\_gyroid\_solid & 6.405 (0.940) & 9.661 (3.193) & 7.726 (2.787) & 10.081 (3.640) & 37.312 (17.303) & \textbf{3.626} (\textbf{0.319}) \\
uniform\_gyroid\_smooth & 0.930 (0.328) & 1.179 (0.303) & 0.729 (0.223) & 1.233 (0.360) & 0.913 (0.328) & \textbf{0.713} (\textbf{0.193}) \\
uniform\_checkerboard & 26.593 (9.282) & 25.723 (8.953) & 22.053 (8.126) & 26.517 (10.257) & 42.139 (20.959) & \textbf{18.598} (\textbf{4.703}) \\
uniform\_fractal & 0.055 (0.019) & 0.071 (0.019) & 0.045 (0.014) & 0.074 (0.022) & 0.051 (0.020) & \textbf{0.041} (\textbf{0.011}) \\
gaussian\_sine\_low & 0.090 (0.027) & 0.171 (0.031) & 0.041 (0.008) & 0.081 (0.014) & 0.062 (0.016) & \textbf{0.024} (\textbf{0.004}) \\
gaussian\_sphere & \textbf{0.000} (\textbf{0.000}) & 14.138 (1.147) & 1.567 (0.441) & 1.888 (0.561) & 6.208 (3.306) & \textbf{0.000} (\textbf{0.000}) \\
clustered\_sine\_low & 0.115 (0.059) & 0.126 (0.021) & 0.025 (0.005) & 0.027 (0.007) & 0.050 (0.015) & \textbf{0.014} (\textbf{0.003}) \\
clustered\_gyroid & 4.663 (0.451) & 6.058 (1.293) & 3.347 (0.846) & 3.364 (1.074) & 37.108 (17.247) & \textbf{0.363} (\textbf{0.023}) \\
exponential\_sine\_low & 0.089 (0.029) & 0.403 (0.060) & 0.060 (0.015) & 0.101 (0.024) & 0.074 (0.024) & \textbf{0.045} (\textbf{0.009}) \\
exponential\_sphere & \textbf{0.000} (\textbf{0.000}) & 2.777 (0.540) & 1.443 (0.418) & 1.933 (0.548) & 6.546 (1.670) & \textbf{0.000} (\textbf{0.000}) \\
grid\_sine\_low & 0.084 (0.029) & 0.179 (0.044) & \textbf{0.073} (0.028) & 0.114 (0.039) & 0.093 (0.032) & 0.075 (\textbf{0.021}) \\
grid\_sphere & \textbf{0.000} (\textbf{0.000}) & 2.992 (0.983) & 1.736 (0.737) & 2.209 (0.820) & 8.661 (2.771) & \textbf{0.000} (\textbf{0.000}) \\
\midrule
\textbf{Average} & 2.651 (0.773) & 4.436 (1.176) & 2.750 (0.963) & 3.453 (1.235) & 9.684 (4.480) & \textbf{1.591} (\textbf{0.369}) \\
\bottomrule
\end{tabular}
\end{table*}

\definecolor{topone}{HTML}{9ECAE1}   % Darker soft blue (1st best)
\definecolor{toptwo}{HTML}{C6DBEF}   % Medium soft blue (2nd best)
\definecolor{topthree}{HTML}{DEEBF7} % Light soft blue  (3rd best)
\begin{table*}[htbp]
\centering
\caption{Neper Polycrystal Microstructure Evaluation Benchmark ($N=100,000$ cells $\rightarrow$ $10,000$ cells, 90\% LOD Reduction). Results are reported as Final MSE (Trajectory AUC) to 3 decimal places. The top three results in each row are highlighted using different shades of blue (\colorbox{topone}{\textbf{1st}}, \colorbox{toptwo}{2nd}, and \colorbox{topthree}{3rd}).}
\label{tab:neper_microstructures_top3}
\begin{tabular}{lcccccc}
\toprule
Microstructure Morphology & Variance & Volume & FPS & Grid & Naive Merge & \textbf{VoroDuce} \\
\midrule
Columnar Additive (Elongated) & 0.527 (0.243) & \cellcolor{toptwo}0.406 (0.173) & \cellcolor{topthree}0.425 (0.190) & 0.430 (0.203) & 0.507 (0.267) & \cellcolor{topone}\textbf{0.350 (0.133)} \\
Dual-Phase Steel (Bimodal)    & 3.139 (1.430) & \cellcolor{toptwo}2.502 (1.433) & \cellcolor{topthree}2.562 (1.122) & 2.727 (1.217) & 2.851 (1.393) & \cellcolor{topone}\textbf{2.011 (0.770)} \\
Equiaxed FCC (Isotropic)      & 1.685 (0.653) & \cellcolor{toptwo}1.084 (0.460) & \cellcolor{topthree}1.136 (0.503) & 1.150 (0.541) & 2.069 (0.794) & \cellcolor{topone}\textbf{0.973 (0.312)} \\
Hexagonal Titanium (HCP)      & 12.773 (5.086) & \cellcolor{toptwo}8.263 (3.555) & \cellcolor{topthree}8.781 (3.911) & 8.835 (4.159) & 14.307 (6.183) & \cellcolor{topone}\textbf{7.814 (2.530)} \\
Rolled Sheet (Anisotropic)    & 1.461 (0.670) & \cellcolor{toptwo}1.105 (0.473) & \cellcolor{topthree}1.172 (0.521) & \cellcolor{topthree}1.172 (0.556) & 1.478 (0.743) & \cellcolor{topone}\textbf{0.968 (0.363)} \\
\midrule
\textbf{Average}              & 3.917 (1.616) & \cellcolor{toptwo}2.672 (1.219) & \cellcolor{topthree}2.815 (1.249) & 2.863 (1.335) & 4.242 (1.876) & \cellcolor{topone}\textbf{2.423 (0.821)} \\
\bottomrule
\end{tabular}
\end{table*}
